Search for charged massive long-lived particles at sqrt(s)= 1.96 TeV

We present a search for charged massive long-lived particles (CMLLPs) that are pair produced in p-pbar collisions at sqrt(s)= 1.96 TeV collected by the D0 experiment at the Fermilab Tevatron collider. Our result is a combination of two searches where either one or both CMLLPs are reconstructed in the detector. We select events with muon-like particles that have both speed and ionization energy loss dE/dx different from muons produced in p-pbar collisions. In the absence of evidence for CMLLPs corresponding to 6.3 fb-1 of integrated luminosity, we set limits on the CMLLP masses in several supersymmetric models, excluding masses below 278 GeV for long-lived gaugino-like charginos, and masses below 244 GeV for long-lived higgsino-like charginos at the 95% C.L. We also set limits on the cross section for pair production of long-lived scalar tau leptons that range from 0.04 pb to 0.008 pb for scalar tau lepton masses of 100 to 300 GeV.

==> acknowledgement.tex <==
% acknowledgement.tex                            26 October 2012 
%
We thank the staffs at Fermilab and collaborating institutions,
and acknowledge support from the
DOE and NSF (USA);
CEA and CNRS/IN2P3 (France);
MON, NRC KI and RFBR (Russia);
CNPq, FAPERJ, FAPESP and FUNDUNESP (Brazil);
DAE and DST (India);
Colciencias (Colombia);
CONACyT (Mexico);
NRF (Korea);
FOM (The Netherlands);
STFC and the Royal Society (United Kingdom);
MSMT and GACR (Czech Republic);
BMBF and DFG (Germany);
SFI (Ireland);
The Swedish Research Council (Sweden);
and
CAS and CNSF (China).
%

